Measurement of the $ZZ$ Production Cross Section in $pp$ Collisions at $\sqrt{s}$ = 13 TeV with the ATLAS Detector

The $ZZ$ production cross section in proton-proton collisions at 13 TeV center-of-mass energy is measured using 3.2 fb$^{-1}$ of data recorded with the ATLAS detector at the Large Hadron Collider. The considered $Z$ boson candidates decay to an electron or muon pair of mass 66-116 GeV. The cross section is measured in a fiducial phase space reflecting the detector acceptance. It is also extrapolated to a total phase space for $Z$ bosons in the same mass range and of all decay modes, giving $16.7^{+2.2}_{-2.0}$(stat.)$^{+0.9}_{-0.7}$(syst.)$^{+1.0}_{-0.7}$(lumi.) pb. The results agree with standard model predictions.

==> ZZEarlyPAPER-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{Measurement of the \ZZ{} Production Cross Section in $\Pproton\Pproton$ Collisions at $\sqrt{s} = 13$~\TeV{} with the ATLAS Detector}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis
% \AtlasAuthorContribute also adds the name to the author list
% Include package latex/atlascontribute to use this
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute
% \usepackage{authblk}
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
% \usepackage{authblk}
% \author{The ATLAS Collaboration%
% \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-007/authorlist.pdf}}
% }

% Date: if not given, uses current date
%\date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{2.6}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{STDM-2015-13}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATL-PHYS-PUB-2014-XXX}
\AtlasNote{ATL-COM-PHYS-2015-1313}

% CERN preprint number
% \PreprintIdNumber{CERN-PH-2014-XX}

% ATLAS date - arXiv submission; to be filled in by the Physics Office
% \AtlasDate{\today}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
\AtlasJournal{Phys.~Rev.~Lett.}
% \AtlasJournalRef{\PLB 789 (2014) 123}
% \AtlasDOI{}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
\input{abstract.tex}
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{Measurement of the \ZZ{} Production Cross Section in $\Pproton\Pproton$ Collisions at $\sqrt{s} = 13$~\TeV{} with the ATLAS Detector}{https://cds.cern.ch/record/2055805}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{8th December 2015}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Maurice Becker, Andrea Bocci, Will Buttinger,
Tiesheng Dai, Denys Denysiuk, Roberto Di Nardo, Cong Geng, Samira
Hassani, Naoki Kimura, Kostas Kordas, Alexandros Marantis, Emily
Nurse, Marc-Andre Pleier, Stefan Richter, Jonatan Rosten, Anton Wolf,
Yusheng Wu, Bing Zhou}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
\AtlasCoverEdBoardMember{Kevin Black~(chair), Walter Hopkins, Laurent Serin}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverEdBoardMember{Reader~2}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-stdm-2015-13-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-stdm-2015-13-editorial-board@cern.ch}


